Counterfactual Fairness with Partially Known Causal Graph

Fair machine learning aims to avoid treating individuals or sub-populations unfavourably based on \textit{sensitive attributes}, such as gender and race. Those methods in fair machine learning that are built on causal inference ascertain discrimination and bias through causal effects. Though causality-based fair learning is attracting increasing attention, current methods assume the true causal graph is fully known. This paper proposes a general method to achieve the notion of counterfactual fairness when the true causal graph is unknown. To be able to select features that lead to counterfactual fairness, we derive the conditions and algorithms to identify ancestral relations between variables on a \textit{Partially Directed Acyclic Graph (PDAG)}, specifically, a class of causal DAGs that can be learned from observational data combined with domain knowledge. Interestingly, we find that counterfactual fairness can be achieved as if the true causal graph were fully known, when specific background knowledge is provided: the sensitive attributes do not have ancestors in the causal graph. Results on both simulated and real-world datasets demonstrate the effectiveness of our method.

==> Pages/Background.tex <==
\section{Background} \label{sec: Preliminary}
In this section, we first review the structural causal model and counterfactual inference. Then we introduce counterfactual fairness criterion and its intuitive implications. 

%%%% Counterfactual Fairness
\subsection{Structural Causal Model and Counterfactual Inference} \label{sec: SCM and CF}
Structural causal model (SCM) \cite{pearl2000models} is a framework to model causal relations between variables. It is defined by a triple $(U,V,F)$, where $V$ are endogeous variables that are observable and $U$ are exogenous variables that are unobserved and cannot be caused by any variable in $V$. The nodes in a causal graph correspond to the variables in $U$ and $V$. The graph is causal in that the directed edge represents the causal effect from the head to tail, which is formalized by the function in $F$ in the SCM, where $F$ is a set of functions ${f_1,...,f_n}$, one for each $V_i \in V$ expressing how $V_i$ is causally dependant on the variables with the edges directed towards $V_i$, which we call 'parent' of $V_i$, i.e., $V_i = f_i(pa_i, U_{pa_i})$, where $pa_i$ is the set of observed variables that is the parent of $V_i$ and $U_{pa_i}$ is the set of unobserved variables that is the parent of $V_i$.

As an interesting type of inference on a SCM, counterfactual inference answers the problems in the counterfactual world. For example, consider in a fairness context, $A$, $Y$ and $X$ represent the sensitive attributes, outcome of interest and other observable attributes respectively. For an individual with $A=a, Y=y$ and $X=x$, a common counterfactual query is, “For this individual, what would have been the value of $Y$ had $A$ taken value $a'$”. The solution for $Y$ can be denoted as $Y_{A \leftarrow a}(u)$ \cite{pearl2000models}. 
%It can be determined by first obtaining the value of the unobserved variable $U$ given the evidence $X=x,A=a,Y=y$ and SCM $\mathcal{M}$, then modifying $M$ by replacing the structural equation for $A$ with the intervention value $A=a'$, and finally, computing the value of any other variables using the new structural equations and the derived exogenous variables $U$.

\subsection{Counterfactual fairness} \label{sec: Counterfactual fairness}
Counterfactual fairness \citep{kusner2017counterfactual} is a fairness criterion based on SCM \citep{pearl2000models}. 

Suppose $A$, $Y$ and $X$ represent the sensitive attributes, outcome of interest and other observable attributes, respectively and the prediction of $Y$ is denoted by $\hat{Y}$. For an individual with $X=x$ and $A=a$, we say the prediction $\hat{Y}$ is counterfactually fair if it would have been the same had $A$ been $a'$ in the counterfactual world as in the real world that $A$ is $a$.

% \subsection{Counterfactual Fairness in Causal DAGs}
% Formally, \citet{kusner2017counterfactual} postulate \cref{def: counterfactual fairness}. This implies \cref{lem: counterfactual fairness implication}, which can be regarded as a guidance to train a counterfactually fair model.

\begin{definition}[Counterfactual fairness] \citep[Definition 5]{kusner2017counterfactual} \label{def: counterfactual fairness}
    We say the prediction $\hat{Y}$ is counterfactually fair if under any context $X =x$ and $A=a$,
    \begin{align}\label{eq: counterfactual fairness}
        &P(\hat{Y}_{A \gets a}(U)=y|X=x,A=a) \\ \nonumber
        &=P(\hat{Y}_{A\gets{a'}}(U)=y|X=x,A=a),    
    \end{align}
    for all $y$ and any value $a'$ attainable by A.
\end{definition}

% Hence, $A$ should not be a cause of $\hat{Y}$ in any individual instance. This implies $\hat{Y}$ can be modeled as a function of the variables not causally dependent on $A$, which can be formulated as $\hat{Y}=f(Z,U)$, where $Z \subseteq X$ and $Z$ will not be altered by $A$, that is $Z_{A \leftarrow a} = Z_{A \leftarrow a'}$. $U$ is any unobserved variables in the causal model. Formally, Lemma \ref{implication} can be regarded as a guidance to train a counterfactually fair model.

The definition of counterfactual fairness immediately suggests the following approach in \cref{lem: counterfactual fairness implication} to design a counterfactually fair model. 

\begin{lemma}\citep[Lemma 1]{kusner2017counterfactual}\label{lem: counterfactual fairness implication}
    Let $\mathcal{G}$ be the causal graph of the given model $(U,V,F)$. Then $\hat{Y}$ will be counterfactually fair if it is a function of the non-descendants of $A$.
\end{lemma}


% \cref{lem: counterfactual fairness implication} provides a feature selection criterion for a counterfactually fair model: selecting the non-descendants of $A$ to predict $Y$ in a causal DAG. Therefore, learning a counterfactually fair prediction can be formalized as the following:

% Suppose we are given the training data $\mathcal{D} \equiv \{(A^{(i)}, X^{(i)}, Y^{(i)})\}$ for $i=1,2,...n$ with $n$ observations. Let $X_{\nsucc{A}}$ denote the non-descendant set of $A$ in the causal graph. In order to learn a fair prediction $\hat{Y}$ for outcome $Y$ accurately, we learn a classifier $\hat{Y} \equiv f_{\theta}{(X_{\nsucc{A}},U)}$ parameterized by $\theta$ by minimizing the loss function $L(\theta) \equiv \sum_{i=1}^{n} \ell(y^{(i)}, f_{\theta}{(x^{(i)}_{\nsucc{A}},U^{(i)})})$ with respect to $\theta$. At the prediction time, for a new observation $(a', x')$, $\hat{y'} = f_{\theta}{(x'_{\nsucc{A}},U'|a', x')}$ \cite{kusner2017counterfactual}.

==> Pages/Introduction.tex <==
\section{Introduction}\label{sec: Introduction}
Increasingly, machine learning is used to make real-life decisions. Accordingly, ethical and societal impacts of machine learning are being called into question. It is desirable to ensure that the learned models do not make discriminatory decisions against any individual or any sub-population group with respect to \textit{sensitive attributes}, e.g., gender, race.

For the purpose of designing a fair model, a statistical fairness criterion is needed and has been the subject of many papers in fair machine learning \cite{grgic2016case, zafar2015learning, dwork2012fairness, hardt2016equality, chouldechova2017fair}. A recent direction in this field is based on the causal framework \cite{pearl2000models}. Causal-based fair learning \cite{zhang2016causal,kilbertus2017avoiding, kusner2017counterfactual, zhang2018fairness, zhang2018equality,nabi2018fair,wu2019pc,chiappa2019path}  treat the presence of causal effect of the sensitive attribute on the decision as discrimination. Among these works, an interpretable and intuitive individual-level fairness criterion is counterfactual fairness \cite{kusner2017counterfactual}. A counterfactually fair decision towards an individual means the same decision would have been taken if the sensitive attribute of this individual were different. \citet{kusner2017counterfactual} also provide an algorithm for achieving counterfactual fairness on a causal DAG. 

However, one limitation for counterfactual fairness in \cite{kusner2017counterfactual} is the assumption of complete knowledge of the causal relationships between variables: the existence of causal relation between any two variables and explicitly specified function of causal relation if it exists. These can be encoded by a Directed Acyclic Graph (DAG) with causal semantics, which is also known as causal DAG \cite{pearl2009causality}. Nevertheless, in practical, complete knowledge of causal relationship (and hence, the causal DAG) is not known due to insufficient understanding of the system under investigation. An obvious path forward is to estimate the causal DAG from observational data. However, without strong assumptions on the data generating process, we can only learn a Markov equivalence class of DAGs that encoding the same set of conditional independencies from data, which can be represented by a completely partially directed acyclic graph (CPDAG) \citep{spirtes2000causation, chickering2002optimal}. With additional background knowledge, we can discern more causal relations, which can be represented by a maximally partially directed acyclic graph (MPDAG) \citep{meek1995causal}, but we still cannot obtain a causal DAG. This motivates our work on fairness with an partially known causal graph that can be learnt directly from data with some background knowledge, MPDAG. CPDAG is a special case of MPDAG without background knowledge, so we deal with MPDAG generally.

In DAGs, if a variable $X$ has a causal path to another variable $Y$, then $X$ is an ancestor of $Y$ and $Y$ is a descendant of $X$. Counterfactual fairness implies the prediction is counterfactual fair if it is a function of the non-descendant of sensitive attributes \cite{kusner2017counterfactual}, which is straightforward to identify in DAGs. 

However, as for a Markov equivalence class of DAGs learnt from observational data with or without background knowledge, with respect to a variable $X$, a variable $Y$ can be either
\begin{itemize}
    \item a \textit{definite descendant} $X$ if $Y$ is a descendant of $X$ in every equivalent DAG,
    \item a \textit{definite non-descendant} of $X$ if $Y$ is a non-descendant of $X$ in every equivalent DAG,
    \item a \textit{possible descendant} of $X$ if $Y$ is neither a definite descendant nor a definite non-descendant of $X$.
\end{itemize}
To achieve counterfactual fairness in MPDAGs, we may select the definite non-descendants and some possible descendants of the sensitive attributes to make prediction, since some possible descendants should be non-descendants in the true DAG. This comes to the core challenge: the identifiability of the ancestral relation between two distinct variables in an MPDAG. 

It has been shown that in an MPDAG, a variable $Y$ is a definite non-descendant of $X$ if and only if there is no possibly causal path from $X$ to $Y$ \cite{perkovic2017interpreting}. There is also a sufficient and necessary graphical criterion \citep[Theorem 1]{fang2021local} to identify whether a variable is a definite descendant of another variable in CPDAGs. However, to the best of our knowledge, such graphical criterion for MPDAGs has not been examined before.

In this paper, under the assumption that there is no selection bias and no latent variable, in order to achieve counterfactual fairness in the Markov equivalence class of DAGs given additional background knowledge, we make the following main contributions:   
\begin{itemize}
    \item We provide a sufficient and necessary graphical criterion to check whether a variable is a definite descendant of another variable on an MPDAG.
    \item Based on the proposed criterion, we give an efficient algorithm to identify ancestral relations between any two variables on an MPDAG.
    \item We propose the first approach for achieving counterfactual fairness on partially known causal graphs, specifically MPDAGs. 
    \item We find that in an MPDAG, counterfactual fairness can be achieved as if the true causal graph is fully known with the assumption that the sensitive attributes can not have ancestors in the causal graph.
%    \item We conduct experiments on two datasets and validate the fairness and prediction accuracy of the proposed model by comparison with other baseline models.
\end{itemize}

The remainder of this paper is organized as follows. In \cref{sec: Preliminary}, we introduce structural causal models and counterfactual fairness. In \cref{sec: Problem Formulation}, we clarify our problem as a feature selection strategy on MPDAGs. In \cref{sec: Identifiability of Ancestral Relations in MPDAGs}, we provide a sufficient and necessary graphical condition to check whether a variable is a definite descendant of another variable in an MPDAG. An efficient algorithm to identify the type of ancestral relation between any two distinct variables is also provided in this section. In \cref{sec: Counterfactual Fairness in MPDAGs}, based on results in \cref{sec: Identifiability of Ancestral Relations in MPDAGs}, we propose an approach to achieve counterfactual fairness in MPDAGs. In \cref{sec: Experiment}, we illustrate our method through experiments on a simulated and a real-world dataset. In \cref{sec: Related Work}, we briefly review the related works. In \cref{sec: Discussion}, we make a conclusion and discuss some possible extensions of our work.
